Shape From Tracing: Towards Reconstructing 3D Object Geometry and SVBRDF Material from Images via Differentiable Path Tracing

Reconstructing object geometry and material from multiple views typically requires optimization. Differentiable path tracing is an appealing framework as it can reproduce complex appearance effects. However, it is difficult to use due to high computational cost. In this paper, we explore how to use differentiable ray tracing to refine an initial coarse mesh and per-mesh-facet material representation. In simulation, we find that it is possible to reconstruct fine geometric and material detail from low resolution input views, allowing high-quality reconstructions in a few hours despite the expense of path tracing. The reconstructions successfully disambiguate shading, shadow, and global illumination effects such as diffuse interreflection from material properties. We demonstrate the impact of different geometry initializations, including space carving, multi-view stereo, and 3D neural networks. Finally, with input captured using smartphone video and a consumer 360? camera for lighting estimation, we also show how to refine initial reconstructions of real-world objects in unconstrained environments.

==> figtex/fig_10view_svbrdf.tex <==
\begin{figure*}[t!]
  \centering
  \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{lc}
        \raisebox{1.5em}{Ground Truth} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_gt_38_GoldFlake.png} &
        \raisebox{1.5em}{Output} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_optim_38_GoldFlake.png}
        \\
        \raisebox{1.5em}{Ground Truth} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_gt_03_Pattern_Tile.png} &
        \raisebox{1.5em}{Output} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_optim_03_Pattern_Tile.png}
        \\
        \raisebox{1.5em}{Ground Truth} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_gt_19_Cobble.png} &
        \raisebox{1.5em}{Output} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_optim_19_Cobble.png}
        \\
        \raisebox{1.5em}{Ground Truth} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_gt_32_asphalt_after_the_rain.png} &
        \raisebox{1.5em}{Output} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_optim_32_asphalt_after_the_rain.png}
        \\
        \raisebox{1.5em}{Ground Truth} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_gt_37_leather_tiles.png} &
        \raisebox{1.5em}{Output} &
        \includegraphics[width=0.8\linewidth]{figs/mat_comp/redner_optim_37_leather_tiles.png}
        \\
    \end{tabular}
\caption{
A collection of 10 input view SVBRDF reconstructions from our planar material capture.
}
\label{fig:mat_recon}
\end{figure*}

==> figtex/fig_materialopt.tex <==
\begin{figure}[t]
  \centering
  \setlength{\tabcolsep}{1pt}
    \begin{tabular}{cc}
        Iteration 1 & Iteration 10  \\
        \includegraphics[width=.49\linewidth]{figs/mesh-colors-iteration-1.png} &
        \includegraphics[width=.49\linewidth]{figs/mesh-colors-iteration-10.png}
        \\
        Iteration 20 & Iteration 100 \\
        \includegraphics[width=.49\linewidth]{figs/mesh-colors-iteration-20.png} &
        \includegraphics[width=.49\linewidth]{figs/mesh-colors-iteration-100.png}
    \end{tabular}
\caption{
Optimizing a mesh colors surface texture to match a target view, starting from an initial solid-gray albedo.
The SIGGRAPH logo resolves more quickly than the blue background because it is significantly brighter than the initial gray albedo, resulting higher losses than other regions and thus stronger gradients.
}
\label{fig:mesh_colors_optimization}
\end{figure}

==> figtex/fig_pix2mesh.tex <==
\begin{figure}[t!]
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccc}
         Input Views & Pixel2Mesh++ &  Our Refinement
         \\
         \includegraphics[width=0.32\linewidth]{figs/P2M/04.png} &
         \includegraphics[width=0.32\linewidth]{figs/P2M/angle1-big.png} &
         \includegraphics[width=0.32\linewidth]{figs/P2M/angle1.png}
         \\
         \includegraphics[width=0.32\linewidth]{figs/P2M/05.png} &
         \includegraphics[width=0.32\linewidth]{figs/P2M/angle2-big.png} &
         \includegraphics[width=0.32\linewidth]{figs/P2M/angle2.png}
         \\
         \includegraphics[width=0.32\linewidth]{figs/P2M/14.png} &
         \includegraphics[width=0.32\linewidth]{figs/P2M/angle3-big.png} &
         \includegraphics[width=0.32\linewidth]{figs/P2M/angle3.png}
         \\
         F1 Score & 63.9 & $\textbf{87.2}$
         \\
    \end{tabular}
    % \includegraphics[width=\linewidth]{figs/placeholder.pdf}
    \caption{Our refinement using a geometry initialization from inputting 3 views from the 3D-R2N2 dataset ~\cite{3Dr2n2} \emph{(Left)} into Pixel2Mesh++~\cite{Pixel2Mesh++}. The deep reconstruction \emph{(Middle)} is quite coarse. We can upsample this initialization using our refinement pipeline recover much more of the object's detail, such as its legs, cushion seams, and sharp edges \emph{(Right)}. Training a neural network on a large number of views is quite inefficient and, if instead using these two methods together, largely unnecessary for retrieving the utmost reconstruction detail. Even the coarse reconstruction from a 3-view deep network is a sufficient geometry initialization for our refinement.  We report the F1 score of both geometry reconstructions with a tolerance of 0.05; our pipeline has significant improvement over its initialization.
    } 
    \label{fig:pixel2mesh}
\end{figure}


==> figtex/fig_shadowart.tex <==

\begin{figure}[t!]
  \centering
  \setlength{\tabcolsep}{1pt}
    \begin{tabular}{cccc}
        %%%%% Top
        %\multicolumn{2}{c}{Shadow Targets }
        \multicolumn{2}{c}{\rule[1.5pt]{2.7em}{0.7pt} Shadow Targets \rule[1.5pt]{2.7em}{0.7pt}} &
        \multicolumn{2}{c}{\rule[1.5pt]{2em}{0.7pt} Rendered Shadows \rule[1.5pt]{2em}{0.7pt}} 
        %Shadow Targets & & Shadow Output
        \\
        \includegraphics[width=.24\linewidth]{figs/shadow_bunny.png} &
        \includegraphics[width=.24\linewidth]{figs/shadow_monkey.png} &

        \includegraphics[width=.24\linewidth]{figs/bunny_shadow_output.png} &
        \includegraphics[width=.24\linewidth]{figs/monkey_shadow_output.png}
        \\
        \end{tabular}
        \begin{tabular}{cc}
        \multicolumn{2}{c}{Optimized Mesh}
        \\
        \includegraphics[width=.48\linewidth]{figs/bunkey-2.png} &
        \includegraphics[width=.48\linewidth]{figs/bunkey-1.png} 
        \\
        \multicolumn{2}{c}{}
        \\
        \includegraphics[width=.48\linewidth]{figs/bunkey-3.png} &
        \includegraphics[width=.48\linewidth]{figs/bunkey-4.png}
        \\
    
    \end{tabular}
\caption{
Shadow art example. The top row shows two target shadows provided to our pipeline cast by meshes of a bunny and a monkey, as well as the shadows cast by the mesh that we produce cast onto two orthogonal white walls. The bottom two rows show the output mesh at multiple views. Due to the regular resampling steps, the mesh maintains a relatively smooth surface despite the sparse target information. Note that because our pipeline produces physically-correct shadows, our targets can contain gradients of soft shadows. In contrast, prior work on computational shadow art assumed binary mask images as shadow targets. Finally, because we optimize through gradient descent and are constrained by only two views, the output mesh converges to a different shape every time , each of which can cast shadows that approximate the targets. 
}
\label{fig:shadow_art}
\end{figure}

==> figtex/fig_simulated_recon.tex <==
\begin{figure}[t!]
  \centering
  \setlength{\tabcolsep}{1pt}
    \begin{tabular}{rcccc}
        & \textbf{Target} & \textbf{Init} & \textbf{Reconstruction} & 
        \\
        \raisebox{1em}{\rotatebox{90}{Render}} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/target/smooth-shade-area-lit-angle1-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/Initialization/flat-shade-area-lit-angle1-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/2-bounce/full-angle1-256.png}
        \includegraphics[width=.23\linewidth]{figs/Buddha/2-bounce/full-angle2-256.png}
        \\
        \raisebox{2em}{\rotatebox{90}{Geo}} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/target/wireframe-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/Initialization/wireframe-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/1-bounce/wireframe-angle1-256.png}
        \includegraphics[width=.23\linewidth]{figs/Buddha/1-bounce/wireframe-angle2-256.png}
        \\
        \raisebox{1em}{\rotatebox{90}{Albedo}} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/target/albedo-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/Initialization/roughness-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/2-bounce/albedo-angle1-256.png}
        \includegraphics[width=.23\linewidth]{figs/Buddha/2-bounce/albedo-angle2-256.png}
        \\
        \raisebox{1em}{\rotatebox{90}{Specular}} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/target/roughness-non-color.png} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/Initialization/roughness-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Buddha/2-bounce/roughness-angle1-non-color.png}
        \includegraphics[width=.23\linewidth]{figs/Buddha/2-bounce/roughness-angle2-non-color.png}
    \end{tabular}
\caption{
Reconstruction of the Buddha model with a nature texture, from a target scene where it was inside the Cornell Box. The optimization used 32 cameras distributed in a Fibonacci sphere, each with 2 light angles, making for a total of 64 images. The image resolution was $128 \times 128$. \revision{Column 2 shows initializations; column 4 shows reconstructions under a novel view.} Fine geometric details on the model's head and robes are captured in our reconstruction, as well as details in the albedo. The target specular texture exhibits some variation; at the expense of some parts of this detail, our specular reconstruction matches the artistic preference of a relatively uniform specular roughness. 
%Toy example comparing local, local + shadows, local + GI on something where color bleeding is really important
%\brad{one camera with a single light angle. resolution was 256 x 256, targets were rendered with 512 samples and 4 maximum bounces. Optimization images were rendered with 512 samples each in the forward and backward passes. texture was limited to a single diffuse albedo color per plane.}
}
\label{fig:buddha_results}
\end{figure}

\begin{figure}[t!]
  \centering
  \setlength{\tabcolsep}{1pt}
    \begin{tabular}{rcccc}
        & \textbf{Target} & \textbf{Init} & \textbf{Reconstruction} & 
        \\
        \raisebox{1em}{\rotatebox{90}{Render}} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/target/smooth-shade-area-lit-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/Initialization/flat-shade-area-lit-angle1-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/2-bounce/full-angle1-256.png}
        \includegraphics[width=.23\linewidth]{figs/Armadillo/2-bounce/full-angle2-256.png}
        \\
        \raisebox{2em}{\rotatebox{90}{Geo}} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/target/wireframe-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/Initialization/wireframe-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/1-bounce/wireframe-angle1-256.png}
        \includegraphics[width=.23\linewidth]{figs/Armadillo/1-bounce/wireframe-angle2-256.png}
        \\
        \raisebox{1em}{\rotatebox{90}{Albedo}} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/target/albedo-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/Initialization/roughness-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/2-bounce/albedo-angle1-256.png}
        \includegraphics[width=.23\linewidth]{figs/Armadillo/2-bounce/albedo-angle2-256.png}
        \\
        \raisebox{1em}{\rotatebox{90}{Specular}} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/target/roughness-non-color.png} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/Initialization/roughness-256.png} &
        \includegraphics[width=.23\linewidth]{figs/Armadillo/2-bounce/roughness-angle1-non-color.png}
        \includegraphics[width=.23\linewidth]{figs/Armadillo/2-bounce/roughness-angle2-non-color.png}
    \end{tabular}
\caption{
Summary of our reconstruction of the Armadillo model inside the Cornell Box, with a blue pattern.
The optimization used 32 cameras distributed in a Fibonacci sphere, each with 2 light angles, making for a total of 64 images. The image resolution was $128 \times 128$. \revision{Column 2 shows initializations; column 4 shows reconstructions under a novel view}
%Toy example comparing local, local + shadows, local + GI on something where color bleeding is really important
%\brad{one camera with a single light angle. resolution was 256 x 256, targets were rendered with 512 samples and 4 maximum bounces. Optimization images were rendered with 512 samples each in the forward and backward passes. texture was limited to a single diffuse albedo color per plane.}
}
\label{fig:armadillo_results}
\end{figure}


==> figtex/fig_svbrdfreconst.tex <==
\begin{figure*}[t]
    \centering
    \setlength{\tabcolsep}{2.0pt}
%   \renewcommand{\arraystretch}{0.5}
    \resizebox{0.55\linewidth}{!}{
    \begin{tabular}{lrcccccc}
        \textbf{} & \textbf{} & \multicolumn{2}{c}{\textbf{Renderings}} &
        \textbf{Normal} & \textbf{Diffuse} & \textbf{Roughness} & \textbf{Specular}
        \\
         \multirow{3}{*}{\raisebox{-3em}{\rotatebox{90}{\emph{Ours}}}} & 
         \raisebox{2.5em}{Ground Truth} & \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_gt/39_testsetMaps/redner_gt_39_testsetMaps_render_0.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_gt/39_testsetMaps/redner_gt_39_testsetMaps_render_8.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_gt/39_testsetMaps/redner_gt_39_testsetMaps_normal.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_gt/39_testsetMaps/redner_gt_39_testsetMaps_diffuse_gamma.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_gt/39_testsetMaps/redner_gt_39_testsetMaps_roughness.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_gt/39_testsetMaps/redner_gt_39_testsetMaps_specular_gamma.png}
        \\
        & \raisebox{2.5em}{Output} & \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_optim/39_testsetMaps/redner_optim_39_testsetMaps_render_0.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_optim/39_testsetMaps/redner_optim_39_testsetMaps_render_8.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_optim/39_testsetMaps/redner_optim_39_testsetMaps_normal.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_optim/39_testsetMaps/redner_optim_39_testsetMaps_diffuse_gamma.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_optim/39_testsetMaps/redner_optim_39_testsetMaps_roughness.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_optim/39_testsetMaps/redner_optim_39_testsetMaps_specular_gamma.png}
        \\
        \multirow{2}{*}{\raisebox{-10em}{\rotatebox{90}{\emph{Deschaintre et al. 2019}}}} & \raisebox{2.5em}{Error} & \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_error/39_testsetMaps/redner_error_39_testsetMaps_render_0.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_error/39_testsetMaps/redner_error_39_testsetMaps_render_8.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_error/39_testsetMaps/redner_error_39_testsetMaps_normal.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_error/39_testsetMaps/redner_error_39_testsetMaps_diffuse_gamma.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_error/39_testsetMaps/redner_error_39_testsetMaps_roughness.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/redner_error/39_testsetMaps/redner_error_39_testsetMaps_specular_gamma.png}
        \\
        & 
        \raisebox{2.5em}{Error} & \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_error/39_testsetMaps/mvsvbrdf_error_39_testsetMaps_render_0.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_error/39_testsetMaps/mvsvbrdf_error_39_testsetMaps_render_9.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_error/39_testsetMaps/mvsvbrdf_error_39_testsetMaps_normal.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_error/39_testsetMaps/mvsvbrdf_error_39_testsetMaps_diffuse_gamma.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_error/39_testsetMaps/mvsvbrdf_error_39_testsetMaps_roughness.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_error/39_testsetMaps/mvsvbrdf_error_39_testsetMaps_specular_gamma.png}
        \\
        & \raisebox{2.5em}{Output} & \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_optim/39_testsetMaps/mvsvbrdf_optim_39_testsetMaps_render_0.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_optim/39_testsetMaps/mvsvbrdf_optim_39_testsetMaps_render_9.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_optim/39_testsetMaps/mvsvbrdf_optim_39_testsetMaps_normal.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_optim/39_testsetMaps/mvsvbrdf_optim_39_testsetMaps_diffuse_gamma.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_optim/39_testsetMaps/mvsvbrdf_optim_39_testsetMaps_roughness.png} &
        \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_optim/39_testsetMaps/mvsvbrdf_optim_39_testsetMaps_specular_gamma.png}
         \\
        % & \raisebox{2.5em}{Ground Truth} &
        % \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_gt/39_testsetMaps/mvsvbrdf_gt_39_testsetMaps_render_0.png} &
        % \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_gt/39_testsetMaps/mvsvbrdf_gt_39_testsetMaps_render_9.png} &
        % \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_gt/39_testsetMaps/mvsvbrdf_gt_39_testsetMaps_normal.png} &
        % \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_gt/39_testsetMaps/mvsvbrdf_gt_39_testsetMaps_diffuse_gamma.png} &
        % \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_gt/39_testsetMaps/mvsvbrdf_gt_39_testsetMaps_roughness.png} &
        % \includegraphics[width=.1\linewidth]{figs/mat_comp/mvsvbrdf_gt/39_testsetMaps/mvsvbrdf_gt_39_testsetMaps_specular_gamma.png}
        \\
        % \midrule
    \end{tabular}
    }
    \hfill
    \resizebox{0.388\linewidth}{!}{
    \begin{tabular}{ccc}
         %& \textbf{MSE} & \textbf{PSNR} & \textbf{SSIM}
         %\\
         & Ours & Deschaintre et al.~2019 \\
         \raisebox{5.5em}{\rotatebox{90}{\textbf{MSE}}} &
         \includegraphics[width=0.33\linewidth]{figs/mat_comp/redner_MSE.png} &
         \includegraphics[width=0.33\linewidth]{figs/mat_comp/mvsvbrdf_MSE.png} \\
         \raisebox{5.5em}{\rotatebox{90}{\textbf{PSNR}}} &
         \includegraphics[width=0.33\linewidth]{figs/mat_comp/redner_PSNR.png} &
         \includegraphics[width=0.33\linewidth]{figs/mat_comp/mvsvbrdf_PSNR.png} \\
         \raisebox{5.5em}{\rotatebox{90}{\textbf{SSIM}}} &
         \includegraphics[width=0.33\linewidth]{figs/mat_comp/redner_SSIM.png} & 
         \includegraphics[width=0.33\linewidth]{figs/mat_comp/mvsvbrdf_SSIM.png} \\
         & \multicolumn{2}{c}{\includegraphics[width=0.38\linewidth]{figs/mat_comp/legend.png}} &
    \end{tabular}
    }
    \vspace{0.3cm}
    \caption{\emph{Left:} SVBRDF reconstruction of a spatially varying wood-like texture given 10 input views. Diffuse and specular albedo maps have a gamma correction of 2.2 applied. Note the comparatively high variation of our material maps despite better re-rendering error. This is due to the lack of a prior and the non-unique optimization landscape--particularly in the intertwined roughness and specular maps. \emph{Right:} Reconstruction metrics plotted as a function of number of input views. Our optimization benefits more from an increased number of views. Note also the stabilization in output quality around 8--10 views. This occurs when it is no longer able to ``cheat'' in the optimization space and perfectly capture particular view points.}
    \label{fig:SVBRDF_qualitative}
\end{figure*}




%%%%%
% JT compressed into qualitative figure
% \begin{figure*}[t!]
%     \centering
%     \setlength{\tabcolsep}{0.0pt}
% %   \renewcommand{\arraystretch}{0.5}
%     \begin{tabular}{lccc}
%          & \textbf{MSE} & \textbf{PSNR} & \textbf{SSIM}
%          \\
%          \raisebox{5.5em}{\rotatebox{90}{Ours}} &
%          \includegraphics[width=0.33\linewidth]{figs/mat_comp/redner_MSE.png} &
%          \includegraphics[width=0.33\linewidth]{figs/mat_comp/redner_PSNR.png} &
%          \includegraphics[width=0.33\linewidth]{figs/mat_comp/redner_SSIM.png}
%          \\
%          \raisebox{1.5em}{\rotatebox{90}{Deschaintre et al. 2019}} &
%          \includegraphics[width=0.33\linewidth]{figs/mat_comp/mvsvbrdf_MSE.png} &
%          \includegraphics[width=0.33\linewidth]{figs/mat_comp/mvsvbrdf_PSNR.png} &
%          \includegraphics[width=0.33\linewidth]{figs/mat_comp/mvsvbrdf_SSIM.png}
%          \\
%     \end{tabular}
%     \includegraphics[width=0.38\linewidth]{figs/mat_comp/legend.png}
%     \caption{SVBRDF reconstruction metrics plotted as a function of number of input views. Our optimization benefits more from an increased number of views. Note also the stabilization in output quality around 8--10 views. This occurs when it is no longer able to "cheat" in the optimization space and perfectly capture particular view points.
%     \loudon{TODO add v2 stats when done}}
%     \label{fig:SVBRDF_plots}
% \end{figure*}
